Stencil scaling for vector-valued PDEs on hybrid grids with applications to generalized Newtonian fluids

Matrix-free finite element implementations for large applications provide an attractive alternative to standard sparse matrix data formats due to the significantly reduced memory consumption. Here, we show that they are also competitive with respect to the run time in the low order case if combined with suitable stencil scaling techniques. We focus on variable coefficient vector-valued partial differential equations as they arise in many physical applications. The presented method is based on scaling constant reference stencils originating from a linear finite element discretization instead of evaluating the bilinear forms on-the-fly. This method assumes the usage of hierarchical hybrid grids, and it may be applied to vector-valued second-order elliptic partial differential equations directly or as a part of more complicated problems. We provide theoretical and experimental performance estimates showing the advantages of this new approach compared to the traditional on-the-fly integration and stored matrix approaches. In our numerical experiments, we consider two specific mathematical models. Namely, linear elastostatics and incompressible Stokes flow. The final example considers a non-linear shear-thinning generalized Newtonian fluid. For this type of non-linearity, we present an efficient approach to compute a regularized strain rate which is then used to define the node-wise viscosity. Depending on the compute architecture, we could observe maximum speedups of 64% and 122% compared to the on-the-fly integration. The largest considered example involved solving a Stokes problem with 12288 compute cores on the state of the art supercomputer SuperMUC-NG.

==> data/memory/roofline.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}[font=\scriptsize]%[scale=\tikzscale]

\begin{axis}[%
width=0.8\textwidth,
height=4cm,
at={(0.769in,0.576in)},
scale only axis,
xmode=log,
xmin=0.01,
xmax=1.5,
xtick={0.01,0.1,1},
xticklabels={{0.01},{ 0.1},{   1}},
xminorticks=true,
xlabel style={font=\color{white!15!black},font=\scriptsize},
xlabel={Arithmetic Intensity [FLOPs/Byte]},
ymode=log,
ymin=0.03,
ymax=200,
ytick={0.1,1,10},
yticklabels={{0.1},{  1},{ 10}},
yminorticks=true,
ylabel style={font=\color{white!15!black},font=\scriptsize},
ylabel={Performance [GFLOPs/s]},
axis background/.style={fill=white},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]


\addplot [color=gray, line width=0.8pt, forget plot, dashed]
table[row sep=crcr]{%
	0.13	36.44\\
	1.5	36.44\\
};
\addplot [color=gray, line width=0.8pt, forget plot, dashed]
table[row sep=crcr]{%
	0.015	4.56\\
	1.5	4.56\\
};


\addplot [color=black, line width=1.2pt, forget plot]
table[row sep=crcr]{%
	0.01	2.8984\\
	0.249758487441347	72.39\\
	1.5	72.39\\
};
\addplot [color=black, line width=1.2pt, forget plot]
table[row sep=crcr]{%
	0.01	0.913\\
	0.792880613362541	72.39\\
	1.5	72.39\\
};
\addplot [color=black, line width=1.2pt, forget plot]
table[row sep=crcr]{%
	0.01	0.2291\\
	3.15975556525535	72.39\\
	1.5	72.39\\
};
\addplot [color=black, line width=1.2pt, forget plot]
table[row sep=crcr]{%
	0.01	0.047\\
	15.4021276595745	72.39\\
	1.5	72.39\\
};

\addplot [color=color1, dashdotted, line width=1.2pt, forget plot]
table[row sep=crcr]{%
	0.01	3.8\\
	0.13	3.8\\
	0.13	0.03\\
};
\addplot [color=color1, line width=1.2pt, draw=none, mark size=4.3pt, mark=diamond*, mark options={solid, fill=color1, color1}]
table[row sep=crcr]{%
	0.13	3.8\\
};
\addlegendentry{Physical scaling}

\addplot [color=color2, dashed, line width=1.2pt, forget plot]
table[row sep=crcr]{%
	0.01	4.89\\
	0.19	4.89\\
	0.19	0.03\\
};
\addplot [color=color2, line width=1.2pt, draw=none, mark size=1.8pt, mark=square*, mark options={solid, fill=color2, color2}]
table[row sep=crcr]{%
	0.19	4.89\\
};
\addlegendentry{Nodal integration}

\addplot [color=color5, line width=1.2pt, forget plot]
table[row sep=crcr]{%
	0.01	0.99\\
	0.11	0.99\\
	0.11	0.03\\
};
\addplot [color=color5, line width=1.2pt, draw=none, mark size=2.5pt, mark=*, mark options={solid, fill=color5, color5}]
table[row sep=crcr]{%
	0.11	0.99\\
};
\addlegendentry{Stored stencil}

\node[right, align=left, rotate=11.5]
at (axis cs:0.011,4) {L1 Bandwidth 289.84 GB/sec};
\node[right, align=left, rotate=11.5]
at (axis cs:0.011,1.3) {L2 Bandwidth 91.30 GB/sec};
\node[right, align=left, rotate=11]
at (axis cs:0.011,0.34) {L3 Bandwidth 22.91 GB/sec};
\node[right, align=left, rotate=11]
at (axis cs:0.011,0.075) {DRAM Bandwidth 4.70 GB/sec};
\node[right, align=left]
at (axis cs:0.25,100.01) {DP Vector FMA 72.39 GFLOPS};

\node[right, align=left]
at (axis cs:0.25,28) {DP Vector Add 36.44 GFLOPS};

\node[right, align=left]
at (axis cs:0.25,6) {DP Scalar Add 4.56 GFLOPS};
\end{axis}
\end{tikzpicture}%

